Positivity bounds on electromagnetic properties of media

We study the constraints imposed on the electromagnetic response of general media by microcausality (commutators of local fields vanish outside the light cone) and positivity of the imaginary parts (the medium can only absorb energy from the external field). The equations of motion for the average electromagnetic field in a medium -- the macroscopic Maxwell equations -- can be derived from the in-in effective action and the effect of the medium is encoded in the electric and magnetic permeabilities $\varepsilon(\omega,|\boldsymbol{k}|)$ and $\mu(\omega,|\boldsymbol{k}|)$. Microcausality implies analyticity of the retarded Green's functions when the imaginary part of the $4$-vector $(\omega,\boldsymbol{k})$ lies in forward light cone. With appropriate assumptions about the behavior of the medium at high frequencies one derives dispersion relations, originally studied by Leontovich. In the case of dielectrics these relations, combined with the positivity of the imaginary parts, imply bounds on the low-energy values of the response, $\varepsilon(0,0)$ and $\mu(0,0)$. In particular the quantities $\varepsilon(0,0)-1$ and $\varepsilon(0,0) - 1/\mu(0,0)$ are constrained to be positive and equal to integrals over the imaginary parts of the response. We discuss various improvements of these bounds in the case of non-relativistic media and with additional assumptions about the UV behavior.

==> tikz/complex.tex <==

\definecolor{ultramarine}{rgb}{0.07, 0.04, 0.56}

\tikzfeynmanset{
	every vertex/.style={ultramarine, dot},
	every particle/.style={blue},
	every blob/.style={draw=green!40!black, pattern color=green!40!black},
}

\feynmandiagram [layered layout, horizontal=a to b]{
a [particle={$A_i$}] -- [boson,opacity=0.3] b [blob] -- [boson,opacity=0.3] d[particle={$A_j$}],
};



==> tikz/feynman2.tex <==

\definecolor{ultramarine}{rgb}{0.07, 0.04, 0.56}

\tikzfeynmanset{
	every vertex/.style={ultramarine, dot},
	every particle/.style={blue},
	every blob/.style={draw=green!40!black, pattern color=green!40!black},
}

%\feynmandiagram [horizontal=a to b] {
	%	a [particle={$A$}] -- [boson] b [blob],
	%	c -- [fermion] b -- [fermion] d, };

%\feynmandiagram [layered layout, horizontal=a to b]{
%	a [particle={$A_i$}] -- [boson] b --[out=125, in=55, loop, min distance=2cm] b -- [boson] c[particle={$A_j$}],
%};

\begin{tikzpicture}[scale=0.9, every node/.style={scale=0.9}]
	\begin{feynman}
		\diagram [horizontal=a to c, layered layout] {
			a [particle={$A_i$}] -- [boson,opacity=0.3] b -- [boson,opacity=0.3] c[particle={$A_j$}],
			%a [particle={$A_i$}] -- [boson] c[particle={$A_j$}],
		};
		\path (b)--++(90:0.45) coordinate (A);
		\draw[color=ultramarine,pattern=north west lines] (A) circle(0.45);
	\end{feynman}
\end{tikzpicture}

%\feynmandiagram [layered layout, horizontal=b to c] { a -- [photon, momentum=\(p\)] b
	%	-- [fermion, half left, looseness=1.5, momentum=\(k\)] c
	%	-- [fermion, half left, looseness=1.5, momentum=\(k-p\)] b, c -- [photon, momentum=\(p\)] d,
	%};

==> tikz/oneloop.tex <==
\tikzfeynmanset{
	%every vertex/.style={red, dot},
	every particle/.style={blue},
	every blob/.style={draw=green!40!black, pattern color=green!40!black},
}

\feynmandiagram [layered layout, horizontal=b to c] { a -- [photon, momentum=$p$] b
	-- [fermion, half left, looseness=1.5, momentum=\(q+p\)] c
	-- [fermion, half left, looseness=1.5, momentum=\(q\)] b, c -- [photon, momentum=\(p\)] d,
};

%\feynmandiagram [layered layout, horizontal=a to b]{
%	a [particle={$A_i$}] -- [boson] b [blob] -- [boson] d[particle={$A_j$}],
%};

%\feynmandiagram [layered layout, horizontal=b to c] { a -- [photon, momentum=\(p\)] b
	%	-- [fermion, half left, looseness=1.5, momentum=\(k\)] c
	%	-- [fermion, half left, looseness=1.5, momentum=\(k-p\)] b, c -- [photon, momentum=\(p\)] d,
	%};

==> tikz/resum.tex <==

\definecolor{ultramarine}{rgb}{0.07, 0.04, 0.56}

\tikzfeynmanset{
	every vertex/.style={ultramarine, dot},
	every particle/.style={blue},
	every blob/.style={draw=green!40!black, pattern color=green!40!black},
}
\feynmandiagram [layered layout, horizontal=a to b]{
	a[particle=] --[opacity=0.3,boson] b [blob] -- [opacity=0.3,boson] c[particle=],
};
%\draw+
%\feynmandiagram [layered layout, horizontal=a2 to b2,small]{
%	a2[particle=] -- [opacity=0.1,boson] b2 [blob] -- [boson] b3 [blob] -- [opacity=0.1,boson] c3[particle=],
%};
%+
%\feynmandiagram [layered layout, horizontal=a3 to b4,small]{
%	a3[particle=] -- [opacity=0.1,boson] b4 [blob] -- [boson] b5 [blob] -- [boson] b6 [blob]--[opacity=0.1,boson] c4[particle=],
%};
%+\dots

%[scale=0.9, every node/.style={scale=0.9}]
%\begin{tikzpicture}
%
%\begin{feynman}
%\diagram [layered layout, horizontal=a to b,small]{
%a[particle=] --[opacity=0.3,boson] b [blob] -- [opacity=0.3,boson] c[particle=],
%};
%\end{feynman}
%\draw (aa) node{$+$};
%[layered layout, horizontal=a3 to b2,small]
%\begin{feynman}
%		\diagram{
%		a3[particle=] -- [opacity=0.1,boson] b2 [blob] -- [boson] b3 [blob] -- [opacity=0.1,boson] c3[particle=],
%	};
%\end{feynman}

%\begin{feynman}
%		\diagram [layered layout, horizontal=a3 to b4,small]{
%	a3[particle=] -- [opacity=0.1,boson] b4 [blob] -- [boson] b5 [blob] -- [boson] b6 [blob]--[opacity=0.1,boson] c4[particle=],
%};
%\end{feynman}


%		\path (b)--++(90:0.45) coordinate (A);
%		\draw[color=ultramarine,pattern=north west lines] (A) circle(0.45);
	
%\end{tikzpicture}

==> tikz/resum2.tex <==

\definecolor{ultramarine}{rgb}{0.07, 0.04, 0.56}

\tikzfeynmanset{
	every vertex/.style={ultramarine, dot},
	every particle/.style={blue},
	every blob/.style={draw=green!40!black, pattern color=green!40!black},
}
%\feynmandiagram [layered layout, horizontal=a to b,small]{
%	a[particle=] --[opacity=0.1,boson] b [blob] -- [opacity=0.1,boson] c[particle=],
%};
%\draw+
\feynmandiagram [layered layout, horizontal=a2 to b2,medium]{
	a2[particle=] -- [opacity=0.3,boson] b2 [blob] -- [boson] b3 [blob] -- [opacity=0.3,boson] c3[particle=],
};
%+
%\feynmandiagram [layered layout, horizontal=a3 to b4,small]{
%	a3[particle=] -- [opacity=0.1,boson] b4 [blob] -- [boson] b5 [blob] -- [boson] b6 [blob]--[opacity=0.1,boson] c4[particle=],
%};
%+\dots

%[scale=0.9, every node/.style={scale=0.9}]
%\begin{tikzpicture}
%\coordinate (a) at (0, 0);
%\coordinate (aa) at (2.1, 0);
%
%\coordinate (a3) at (2.2, 0);
%\coordinate (b3) at (2.5, 0);
%\coordinate (bb3) at (4, 0);
%\coordinate (c3) at (5, 0);

%\begin{feynman}
%\diagram [layered layout, horizontal=a to b,small]{
%a[particle=] --[opacity=0.3,boson] b [blob] -- [opacity=0.3,boson] c[particle=],
%};
%\end{feynman}
%\draw (aa) node{$+$};
%[layered layout, horizontal=a3 to b2,small]
%\begin{feynman}
%		\diagram{
%		a3[particle=] -- [opacity=0.1,boson] b2 [blob] -- [boson] b3 [blob] -- [opacity=0.1,boson] c3[particle=],
%	};
%\end{feynman}

%\begin{feynman}
%		\diagram [layered layout, horizontal=a3 to b4,small]{
%	a3[particle=] -- [opacity=0.1,boson] b4 [blob] -- [boson] b5 [blob] -- [boson] b6 [blob]--[opacity=0.1,boson] c4[particle=],
%};
%\end{feynman}


%		\path (b)--++(90:0.45) coordinate (A);
%		\draw[color=ultramarine,pattern=north west lines] (A) circle(0.45);
	
%\end{tikzpicture}

==> tikz/resum3.tex <==

\definecolor{ultramarine}{rgb}{0.07, 0.04, 0.56}

\tikzfeynmanset{
	every vertex/.style={ultramarine, dot},
	every particle/.style={blue},
	every blob/.style={draw=green!40!black, pattern color=green!40!black},
}
%\feynmandiagram [layered layout, horizontal=a to b,small]{
%	a[particle=] --[opacity=0.1,boson] b [blob] -- [opacity=0.1,boson] c[particle=],
%};
%\draw+
%\feynmandiagram [layered layout, horizontal=a2 to b2,small]{
%	a2[particle=] -- [opacity=0.1,boson] b2 [blob] -- [boson] b3 [blob] -- [opacity=0.1,boson] c3[particle=],
%};
%+
\feynmandiagram [layered layout, horizontal=a3 to b4,medium]{
	a3[particle=] -- [opacity=0.3,boson] b4 [blob] -- [boson] b5 [blob] -- [boson] b6 [blob]--[opacity=0.3,boson] c4[particle=],
};
%+\dots

%[scale=0.9, every node/.style={scale=0.9}]
%\begin{tikzpicture}
%\coordinate (a) at (0, 0);
%\coordinate (aa) at (2.1, 0);
%
%\coordinate (a3) at (2.2, 0);
%\coordinate (b3) at (2.5, 0);
%\coordinate (bb3) at (4, 0);
%\coordinate (c3) at (5, 0);
%
%\begin{feynman}
%\diagram [layered layout, horizontal=a to b,small]{
%a[particle=] --[opacity=0.3,boson] b [blob] -- [opacity=0.3,boson] c[particle=],
%};
%\end{feynman}
%\draw (aa) node{$+$};
%[layered layout, horizontal=a3 to b2,small]
%\begin{feynman}
%		\diagram{
%		a3[particle=] -- [opacity=0.1,boson] b2 [blob] -- [boson] b3 [blob] -- [opacity=0.1,boson] c3[particle=],
%	};
%\end{feynman}

%\begin{feynman}
%		\diagram [layered layout, horizontal=a3 to b4,small]{
%	a3[particle=] -- [opacity=0.1,boson] b4 [blob] -- [boson] b5 [blob] -- [boson] b6 [blob]--[opacity=0.1,boson] c4[particle=],
%};
%\end{feynman}


%		\path (b)--++(90:0.45) coordinate (A);
%		\draw[color=ultramarine,pattern=north west lines] (A) circle(0.45);
	
%\end{tikzpicture}

==> tikz/resumfrac1.tex <==

\definecolor{ultramarine}{rgb}{0.07, 0.04, 0.56}

\tikzfeynmanset{
	every vertex/.style={ultramarine, dot},
	every particle/.style={blue},
	every blob/.style={draw=green!40!black, pattern color=green!40!black},
}
%\feynmandiagram [layered layout, horizontal=a to b,small]{
%	a[particle=] --[opacity=0.1,boson] b [blob] -- [opacity=0.1,boson] c[particle=],
%};
%\draw+
%\feynmandiagram [layered layout, horizontal=a2 to b2,small]{
%	a2[particle=] -- [opacity=0.1,boson] b2 [blob] -- [boson] b3 [blob] -- [opacity=0.1,boson] c3[particle=],
%};
%+
\feynmandiagram [layered layout, horizontal=a3 to b4,small]{
	a3[particle=] -- [opacity=0.0,boson] b4 [blob] --[opacity=0.0,boson] c4[particle=],
};
%+\dots

%[scale=0.9, every node/.style={scale=0.9}]
%\begin{tikzpicture}
%\coordinate (a) at (0, 0);
%\coordinate (aa) at (2.1, 0);
%
%\coordinate (a3) at (2.2, 0);
%\coordinate (b3) at (2.5, 0);
%\coordinate (bb3) at (4, 0);
%\coordinate (c3) at (5, 0);
%
%\begin{feynman}
%\diagram [layered layout, horizontal=a to b,small]{
%a[particle=] --[opacity=0.3,boson] b [blob] -- [opacity=0.3,boson] c[particle=],
%};
%\end{feynman}
%\draw (aa) node{$+$};
%[layered layout, horizontal=a3 to b2,small]
%\begin{feynman}
%		\diagram{
%		a3[particle=] -- [opacity=0.1,boson] b2 [blob] -- [boson] b3 [blob] -- [opacity=0.1,boson] c3[particle=],
%	};
%\end{feynman}

%\begin{feynman}
%		\diagram [layered layout, horizontal=a3 to b4,small]{
%	a3[particle=] -- [opacity=0.1,boson] b4 [blob] -- [boson] b5 [blob] -- [boson] b6 [blob]--[opacity=0.1,boson] c4[particle=],
%};
%\end{feynman}


%		\path (b)--++(90:0.45) coordinate (A);
%		\draw[color=ultramarine,pattern=north west lines] (A) circle(0.45);
	
%\end{tikzpicture}

==> tikz/resumfrac2.tex <==

\definecolor{ultramarine}{rgb}{0.07, 0.04, 0.56}

\tikzfeynmanset{
	every vertex/.style={ultramarine, dot},
	every particle/.style={blue},
	every blob/.style={draw=green!40!black, pattern color=green!40!black},
}
%\feynmandiagram [layered layout, horizontal=a to b,small]{
%	a[particle=] --[opacity=0.1,boson] b [blob] -- [opacity=0.1,boson] c[particle=],
%};
%\draw+
\feynmandiagram [layered layout, horizontal=a2 to b2,small]{
	a2[particle=] -- [boson] b2 [blob] -- [opacity=0.0,boson] c3[particle=],
};
%\feynmandiagram [layered layout, horizontal=a3 to b4,small]{
%	a3[particle=] -- [opacity=0.0,boson] b4 [blob] --[opacity=0.0,boson] c4[particle=],
%};
%+\dots

%[scale=0.9, every node/.style={scale=0.9}]
%\begin{tikzpicture}
%\coordinate (a) at (0, 0);
%\coordinate (aa) at (2.1, 0);
%
%\coordinate (a3) at (2.2, 0);
%\coordinate (b3) at (2.5, 0);
%\coordinate (bb3) at (4, 0);
%\coordinate (c3) at (5, 0);
%
%\begin{feynman}
%\diagram [layered layout, horizontal=a to b,small]{
%a[particle=] --[opacity=0.3,boson] b [blob] -- [opacity=0.3,boson] c[particle=],
%};
%\end{feynman}
%\draw (aa) node{$+$};
%[layered layout, horizontal=a3 to b2,small]
%\begin{feynman}
%		\diagram{
%		a3[particle=] -- [opacity=0.1,boson] b2 [blob] -- [boson] b3 [blob] -- [opacity=0.1,boson] c3[particle=],
%	};
%\end{feynman}

%\begin{feynman}
%		\diagram [layered layout, horizontal=a3 to b4,small]{
%	a3[particle=] -- [opacity=0.1,boson] b4 [blob] -- [boson] b5 [blob] -- [boson] b6 [blob]--[opacity=0.1,boson] c4[particle=],
%};
%\end{feynman}


%		\path (b)--++(90:0.45) coordinate (A);
%		\draw[color=ultramarine,pattern=north west lines] (A) circle(0.45);
	
%\end{tikzpicture}
